Energy-Efficient Power Allocation in Cell-Free Massive MIMO via Graph Neural Networks

CF-mMIMO systems are a promising solution to enhance the performance in 6G wireless networks. Its distributed nature of the architecture makes it highly reliable, provides sufficient coverage and allows higher performance than cellular networks. EE is an important metric that reduces the operating costs and also better for the environment. In this work, we optimize the downlink EE performance with MRT precoding and power allocation. Our aim is to achieve a less complex, distributed and scalable solution. To achieve this, we apply unsupervised ML with permutation equivariant architecture and use a non-convex objective function with multiple local optima. We compare the performance with the centralized and computationally expensive SCA. The results indicate that the proposed approach can outperform the baseline with significantly less computation time.

==> support-regularization.tex <==
\section{Support Regularization}
Support regularization plays a crucial role in the success of the training because it helps to escape the local optima while ensuring global optimum is still in the support of $[\mathbf{a},\mathbf{b}]$.
This idea was introduced in one of our previous works as entropy regularization~\cite{Peng2023} for \gls{ee} maximization under power constraints for interference networks.
From our experiments, it was clear that support regularization was sufficient for this problem and produced similar results to entropy regularization. 
The only difference being the regularization is much faster since the regularization term is updated linearly rather than in a logarithmic way.
It is a common practice to change the problem into dual form to optimize the regularization factor~\cite{haarnoja2018soft}.
However, since it is very difficult to obtain the infimum of the Lagrangian of our complicated objective function (unlike the canonical definition of the dual problem),
there is no guarantee of convexity of the dual problem,
which would be a fatal disadvantage in the considered problem.
A simple heuristic approach was proposed in~\cite{Peng2023} to tune $\kappa$. 
Let $\kappa_i$ be the $\kappa$ in iteration~$i$ of the gradient ascent optimization.
$\kappa_i = 0$ for $i \leq h$,
where $h$ is a hyper-parameter for constant $\kappa$.
For $i > h$,
$\kappa$ is computed as
\begin{equation}
    \kappa_{i + 1} =
    \begin{cases}
    \kappa_i + \Delta\kappa & \text{if}\; \sum_{j = 1}^{h} \psi_{i - j} / h \leq \psi_i \\
    \max(0, \kappa_t - \Delta\kappa / 2) & \text{otherwise,}\\
    \end{cases}
    \label{eq:updating_kappa}
\end{equation}
where $\Delta\kappa$ is a constant small learning rate.
The intuition behind \eqref{eq:updating_kappa} is that we carefully increase $\kappa$ if the entropy does not reduce (case~1)
and decrease $\kappa$ otherwise such that $\kappa$ is not too big to make $\mathbf{a}$ or $\mathbf{b}$ cross the global optimum (case~2).


